RLIE: Rule Generation with Logistic Regression, Iterative Refinement, and Evaluation for Large Language Models

Large Language Models (LLMs) can propose rules in natural language, sidestepping the need for a predefined predicate space in traditional rule learning. Yet many LLM-based approaches ignore interactions among rules, and the opportunity to couple LLMs with probabilistic rule learning for robust inference remains underexplored. We present RLIE, a unified framework that integrates LLMs with probabilistic modeling to learn a set of weighted rules. RLIE has four stages: (1) Rule generation, where an LLM proposes and filters candidates; (2) Logistic regression, which learns probabilistic weights for global selection and calibration; (3) Iterative refinement, which updates the rule set using prediction errors; and (4) Evaluation, which compares the weighted rule set as a direct classifier with methods that inject rules into an LLM. We evaluate multiple inference strategies on real-world datasets. Applying rules directly with their learned weights yields superior performance, whereas prompting LLMs with the rules, weights, and logistic-model outputs surprisingly degrades accuracy. This supports the view that LLMs excel at semantic generation and interpretation but are less reliable for precise probabilistic integration. RLIE clarifies the potential and limitations of LLMs for inductive reasoning and couples them with classic probabilistic rule combination methods to enable more reliable neuro-symbolic reasoning.

==> tables/combined_results.tex <==
% \resizebox{\textwidth}{!}{% <--- 设置宽度为文本宽度，高度自动(!)
% \begin{tabular}{c|l|cccccc}
% \hline
% & \textbf{Method} & \textbf{Reviews} & \textbf{Dreaddit} & \textbf{Headlines} & \textbf{Citations} & \textbf{LLM Detect} & \textbf{Retweets} \\
% \hline
% \multirow{5}{*}{\rotatebox{90}{\textbf{Accuracy}}} & Zero-shot Inference & 55.11±0.18 & 62.00±0.88 & \underline{63.22±2.52} & 56.25±0.00 & 56.11±0.38 & \underline{65.56±2.34} \\
% & Zero-shot Generation & 63.89±5.50 & 64.33±2.19 & 53.67±1.20 & \underline{58.33±3.61} & 52.44±1.07 & 57.67±2.40 \\
% & IO Refinement & \underline{64.11±5.52} & \textbf{74.89±3.47} & 59.67±3.51 & 48.96±1.80 & \textbf{60.33±17.32} & 62.44±0.69 \\
% & HypoGeniC & 58.00±6.35 & 65.67±0.00 & 60.78±3.27 & 47.92±7.22 & 54.56±4.43 & \underline{65.56±2.12} \\
% & RLIE (Ours) & \textbf{71.00±0.67} & \underline{69.11±1.17} & \textbf{65.56±1.50} & \textbf{59.38±3.12} & \underline{58.67±2.65} & \textbf{65.78±1.71} \\
% \hline\hline
% \multirow{5}{*}{\rotatebox{90}{\textbf{F1 Score}}} & Zero-shot Inference & 50.36±2.30 & 55.67±2.30 & \underline{62.70±2.53} & 36.00±0.00 & 46.77±0.68 & 64.69±2.20 \\
% & Zero-shot Generation & \underline{63.41±6.09} & 59.17±2.84 & 53.10±0.66 & 42.56±7.04 & 39.68±1.58 & 57.64±2.42 \\
% & IO Refinement & 62.03±8.45 & \textbf{73.98±3.59} & 59.21±3.23 & \underline{45.66±2.19} & \textbf{54.00±22.42} & 62.30±0.66 \\
% & HypoGeniC & 56.82±6.29 & 60.57±0.61 & 59.56±3.82 & 41.96±3.40 & 44.17±8.75 & \textbf{65.49±2.17} \\
% & RLIE (Ours) & \textbf{70.81±0.59} & \underline{65.94±1.25} & \textbf{65.38±1.44} & \textbf{49.08±2.84} & \underline{52.10±4.51} & \underline{65.45±1.41} \\
% \hline
% \end{tabular}
% }

\textbf{\resizebox{\textwidth}{!}{% <--- 设置宽度为文本宽度，高度自动(!)
\begin{tabular}{c|l|cccccc}
\hline
& \textbf{Method} & \textbf{Reviews} & \textbf{Dreaddit} & \textbf{Headlines} & \textbf{Citations} & \textbf{LLM Detect} & \textbf{Retweets} \\
\hline
\multirow{6}{*}{\rotatebox{90}{\textbf{Accuracy}}} 
& Zero-shot Inference & 55.11±0.18 & 62.00±0.88 & \underline{63.22±2.52} & 56.25±0.00 & 56.11±0.38 & \underline{65.56±2.34} \\
& Zero-shot Generation & 63.89±5.50 & 64.33±2.19 & 53.67±1.20 & \underline{58.33±3.61} & 52.44±1.07 & 57.67±2.40 \\
& IO Refinement & 64.11±5.52 & \underline{74.89±3.47} & 59.67±3.51 & 48.96±1.80 & \underline{60.33±17.32} & 62.44±0.69 \\
& HypoGeniC & 58.00±6.35 & 65.67±0.00 & 60.78±3.27 & 47.92±7.22 & 54.56±4.43 & \underline{65.56±2.12} \\
% & Zhong et al. & \underline{66.20} & \textbf{75.40} & 48.20 & 58.10 & \textbf{84.90} & 50.00 \\
& RLIE (Ours) & \textbf{71.00±0.67} & 69.11±1.17 & \textbf{65.56±1.50} & \textbf{59.38±3.12} & 58.67±2.65 & \textbf{65.78±1.71} \\
\hline\hline
\multirow{6}{*}{\rotatebox{90}{\textbf{F1 Score}}} 
& Zero-shot Inference & 50.36±2.30 & 55.67±2.30 & \underline{62.70±2.53} & 36.00±0.00 & 46.77±0.68 & 64.69±2.20 \\
& Zero-shot Generation & 63.41±6.09 & 59.17±2.84 & 53.10±0.66 & 42.56±7.04 & 39.68±1.58 & 57.64±2.42 \\
& IO Refinement & 62.03±8.45 & \underline{73.98±3.59} & 59.21±3.23 & 45.66±2.19 & \underline{54.00±22.42} & 62.30±0.66 \\
& HypoGeniC & 56.82±6.29 & 60.57±0.61 & 59.56±3.82 & 41.96±3.40 & 44.17±8.75 & \textbf{65.49±2.17} \\
& Zhong et al. & \underline{65.90} & \textbf{75.00} & 44.10 & \textbf{54.70} & \textbf{84.60} & 52.10 \\
& RLIE (Ours) & \textbf{70.81±0.59} & 65.94±1.25 & \textbf{65.38±1.44} & \underline{49.08±2.84} & 52.10±4.51 & \underline{65.45±1.41} \\
\hline
\end{tabular}
}

==> tables/inference_comparison.tex <==
\resizebox{\textwidth}{!}{% <--- 设置宽度为文本宽度，高度自动(!)
\begin{tabular}{c|l|cccccc}
\hline
& \textbf{Inference Strategy} & \textbf{Reviews} & \textbf{Dreaddit} & \textbf{Headlines} & \textbf{Citations} & \textbf{LLM Detect} & \textbf{Retweets} \\
\hline
\multirow{4}{*}{\rotatebox{90}{\textbf{Accuracy}}}
& Regression Only & \textbf{71.00±0.67} & \textbf{69.11±1.17} & \textbf{65.56±1.50} & \underline{59.38±3.12} & \textbf{58.67±2.65} & \textbf{65.78±1.71} \\
& LLM Evaluation & \underline{65.22±2.67} & 64.56±0.51 & 61.33±3.06 & \textbf{60.42±1.80} & 55.22±2.12 & 61.00±3.06 \\
& LLM + Linear Regression & 64.67±2.33 & 67.56±2.50 & 61.89±3.02 & \textbf{60.42±1.80} & 54.11±2.22 & \underline{62.22±3.56} \\
& LLM + Linear + Label & 64.67±2.60 & \underline{69.00±1.33} & \underline{65.33±1.86} & \underline{59.38±3.12} & \underline{56.67±3.51} & 60.22±3.56 \\
\hline\hline
\multirow{4}{*}{\rotatebox{90}{\textbf{F1 Score}}}
& Regression Only & \textbf{70.81±0.59} & \textbf{65.94±1.25} & \textbf{65.38±1.44} & \textbf{49.08±2.84} & \textbf{52.10±4.51} & \textbf{65.45±1.41} \\
& LLM Evaluation & \underline{64.52±3.19} & 59.57±0.94 & 60.88±3.18 & \underline{48.62±1.19} & 46.82±5.32 & \underline{60.33±3.13} \\
& LLM + Linear Regression & 63.87±3.05 & 63.73±3.72 & 61.71±2.93 & 47.11±3.38 & 44.76±4.62 & 59.68±4.45 \\
& LLM + Linear + Label & 63.80±2.87 & \underline{65.79±1.51} & \underline{65.16±1.78} & \textbf{49.08±2.84} & \underline{48.70±6.05} & 57.38±4.84 \\
\hline
\end{tabular}
}
